Fast Lane-Level Intersection Estimation using Markov Chain Monte Carlo Sampling and B-Spline Refinement

Estimating the current scene and understanding the potential maneuvers are essential capabilities of automated vehicles. Most approaches rely heavily on the correctness of maps, but neglect the possibility of outdated information. We present an approach that is able to estimate lanes without relying on any map prior. The estimation is based solely on the trajectories of other traffic participants and is thereby able to incorporate complex environments. In particular, we are able to estimate the scene in the presence of heavy traffic and occlusions. The algorithm first estimates a coarse lane-level intersection model by Markov chain Monte Carlo sampling and refines it later by aligning the lane course with the measurements using a non-linear least squares formulation. We model the lanes as 1D cubic B-splines and can achieve error rates of less than 10cm within real-time.

==> figures/tikz/colors.tex <==
\definecolor{fzi-darkgreen}{RGB}{0,176,109}
\definecolor{fzi-green}{RGB}{0,108,66}
\definecolor{fzi-lightgreen}{RGB}{115,154,131}
\definecolor{fzi-brightgreen}{RGB}{0,180,111}
\definecolor{fzi-happygreen}{RGB}{146,208,80}
\definecolor{fzi-superlightgreen}{RGB}{191,205,196}
\definecolor{fzi-red}{RGB}{255,0,71}
\definecolor{fzi-blue}{RGB}{0,100,163}
\definecolor{fzi-lightblue}{RGB}{136,195,230}
\definecolor{fzi-yellow}{RGB}{250,187,8}

==> figures/tikz/lane_model_spline_explanation.tex <==

    \begin{tikzpicture}[
      rotate=180,
      scale=0.6,
      arrow/.style={thin,<->,shorten >=1pt,shorten <=1pt,>=stealth},
      larrow/.style={thick,<-,>=stealth},
      rarrow/.style={thick,->,>=stealth}
    ]
\foreach \y in {-1,0}{
	\draw [thin] plot [smooth] coordinates { (-1, \y)(1,\y) (3,\y) (5,\y) (7,\y)};
}
    
\foreach \sign in {1}{
	\foreach \x in {0.5,1.5,2.5}{
		\draw [thin] plot [smooth] coordinates { 
			  (\sign*\x,\sign*4)       
		      (\sign*\x+\sign*0.1*1*1,\sign*4-\sign*1.88*1) 
		      (\sign*\x+\sign*0.1*2*2,\sign*4-\sign*1.88*2)
		      (\sign*\x+\sign*0.1*3*3,\sign*4-\sign*1.88*3)
%			  (\sign*\x+\sign*0.1*4*4,\sign*4-\sign*1.88*4) 
		};
	}
}

% Trajectories

\draw [rarrow,fzi-happygreen, dotted, thick] plot [smooth] coordinates { (7,-0.5) (4.5,-0.45) (2.65,0.15) (2.1,2) (2,2.5) (2,4)};
\node at (7.2,-0.5) {\scriptsize A};

\draw [larrow,fzi-yellow, dotted, thick] plot [smooth] coordinates {
%	(0.5+1.5,1*4)       
	(0.5+1.5+1*0.1*1*1,1*4-1*1.88*1) 
	(0.5+1.5+1*0.1*2*2,1*4-1*1.88*2)
	(0.5+1.5+1*0.1*3*3,1*4-1*1.88*3)
%	(0.5+1.5+1*0.1*4*4,1*4-1*1.88*4) 
};
\draw [larrow,fzi-red, dotted, thick] plot [smooth] coordinates {
	(-0.5+1.5,1*4)       
	(-0.5+1.5+1*0.1*1*1,1*4-1*1.88*1) 
	(-0.5+1.5+1*0.1*2*2,1*4-1*1.88*2)
	(-0.5+1.5+1*0.1*3*3,1*4-1*1.88*3)
%	(-0.5+1.5+1*0.1*4*4,1*4-1*1.88*4) 
};
\node at (2,-2) {\scriptsize B};
\node at (3,-2) {\scriptsize C};

% Distance
\draw [larrow, thick, fzi-blue] (1.1,2.5)  -- (2,2.5);
\node at (1.5,2.8) {\tiny $d_\perp$};


%Turning Lanes
\draw [thin] plot [smooth] coordinates { (6.5,0) (4.5,0.05) (3,0.5) (2.59,2) (2.5,4)};
\draw [thin] plot [smooth] coordinates {(6.5,-1) (4.5,-0.95) (2.35,-0.15) (1.6,2) (1.5,4)};    

% Coords
\draw [larrow,fzi-happygreen, thick] (2+3,3.1) -- (2+4.5,1.7) ;
\draw [larrow,fzi-happygreen, thick] (5.1,0.29) -- (2+4.5,1.7) ;
\node[color=fzi-happygreen] at (4.9,3.1) {\tiny x};
\node[color=fzi-happygreen] at (5,0.29) {\tiny y};

\draw [larrow,fzi-red, thick] (6.1,3.585) -- (2+4.5,1.7) ;
\draw [larrow,fzi-red, thick] (4.55,1.24) -- (2+4.5,1.7) ; 
\node[color=fzi-red] at (6.1,3.685) {\tiny x};
\node[color=fzi-red] at (4.45,1.24) {\tiny y};

\draw [larrow,thick] (5.5,1.7) -- (2+4.5,1.7) ;
\draw [larrow,thick] (6.5,0.7) -- (2+4.5,1.7) ; 
\node at (5.4,1.7) {\tiny x};
\node at (6.5,0.6) {\tiny y};

% Arrows
\draw [rarrow,thick,fzi-happygreen] (4.5,-0.45) -- (4.15,-0.8) ;
\draw [rarrow,thick,fzi-happygreen] (2.65,0.15) -- (2.3,-0.2) ;
\draw [rarrow,thick,fzi-happygreen] (2.1,2) -- (1.75,1.65) ;

\draw [rarrow,thick,fzi-red] (-0.5+1.5+1*0.1*1*1,1*4-1*1.88*1)  -- (-0.5+1.5+1*0.1*1*1-0.48,1*4-1*1.88*1-0.11) ;
\draw [rarrow,thick,fzi-red] (-0.5+1.5+1*0.1*2*2,1*4-1*1.88*2)  -- (-0.5+1.5+1*0.1*2*2-0.48,1*4-1*1.88*2-0.11) ;
\draw [rarrow,thick,fzi-red] (-0.5+1.5+1*0.1*3*3,1*4-1*1.88*3)  -- (-0.5+1.5+1*0.1*3*3-0.48,1*4-1*1.88*3-0.11) ;

%\draw [rarrow,thick,fzi-blue] (0.5+1.5+1*0.1*1*1,1*4-1*1.88*1)  -- (0.5+1.5+1*0.1*1*1-0.48,1*4-1*1.88*1-0.11) ;
%\draw [rarrow,thick,fzi-blue] (0.5+1.5+1*0.1*2*2,1*4-1*1.88*2)  -- (0.5+1.5+1*0.1*2*2-0.48,1*4-1*1.88*2-0.11) ;
%\draw [rarrow,thick,fzi-blue] (0.5+1.5+1*0.1*3*3,1*4-1*1.88*3)  -- (0.5+1.5+1*0.1*3*3-0.48,1*4-1*1.88*3-0.11) ;

% Variables
%\draw [ultra thin] (7, -0.5) -- (7, -1);
%\node at (7.2, -0.75) {\tiny $w$};

\node at (6,-0.25) {\tiny $f_A$};
\node at (1.35,-0.75) {\tiny $f_B$};
%\node at (3,-0.79) {\tiny $f_C$};

    \end{tikzpicture}


==> figures/tikz/lane_model_withtraj.tex <==

    \begin{tikzpicture}[
      scale=0.6,
      arrow/.style={thin,<->,shorten >=1pt,shorten <=1pt,>=stealth},
      larrow/.style={thick,<-,>=stealth},
      rarrow/.style={thick,->,>=stealth}
    ]
\foreach \y in {1.5,0.5,-0.5,-1.5}{
	\draw [thick] plot [smooth] coordinates { (-7,\y) (-5,\y) (-3,\y) (-1,\y) (1,\y) (3,\y) (5,\y) (7,\y)};
}
    
\foreach \sign in {-1,1}{
	\foreach \x in {0.5,1.5,2.5}{
		\draw [thick] plot [smooth] coordinates { 
			  (\sign*\x,\sign*4)       
		      (\sign*\x+\sign*0.1*1*1,\sign*4-\sign*1.88*1) 
		      (\sign*\x+\sign*0.1*2*2,\sign*4-\sign*1.88*2)
		      (\sign*\x+\sign*0.1*3*3,\sign*4-\sign*1.88*3)
			  (\sign*\x+\sign*0.1*4*4,\sign*4-\sign*1.88*4) 
		};
	}
}

% Trajectories
\draw [fzi-red, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, ] plot [smooth] coordinates {
	(0.5+1.5,1*4)       
	(0.5+1.5+1*0.1*1*1,1*4-1*1.88*1) 
	(0.5+1.5+1*0.1*2*2,1*4-1*1.88*2)
	(0.5+1.5+1*0.1*3*3,1*4-1*1.88*3)
	(0.5+1.5+1*0.1*4*4,1*4-1*1.88*4) 
};

\draw [fzi-happygreen, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round] plot [smooth] coordinates {
	(0.5+-1.5,-1*4)       
	(0.5+-1.5+-1*0.1*1*1,-1*4--1*1.88*1) 
	(0.5+-1.5+-1*0.1*2*2,-1*4--1*1.88*2)
	(0.5+-1.5+-1*0.1*3*3,-1*4--1*1.88*3)
	(0.5+-1.5+-1*0.1*4*4,-1*4--1*1.88*4) 
};

\draw [fzi-yellow, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round] plot [smooth] coordinates { (6.5,1) (4.5,1.05) (2.65,1.65) (2,3.5) (1.9,4) };

\draw [fzi-lightblue, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, ] plot [smooth] coordinates {(-7,-1) (-5,-1) (-3,-1) (-1,-1) (1,-1) (3,-1) (5,-1) (7,-1)};


%Turning Lanes
\draw [thick] plot [smooth] coordinates { (6.5,1.5) (4.5,1.55) (3,2) (2.55,3.5) (2.5,4)};
\draw [thick] plot [smooth] coordinates {(6.5,0.5) (4.5,0.55) (2.35,1.35) (1.55,3.5) (1.5,4)};    

\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-7,-0.5) rectangle (-3,0.5);

\draw [rarrow] (-5,-1) -- (-4,-1);\draw [larrow] (-5,1) -- (-4,1);
\draw [larrow] (5,-1) -- (4,-1);\draw [rarrow] (5,1) -- (4,1);
\draw [larrow] (5,0) -- (4,0);

\draw [larrow] (1,3) -- (1,2);\draw [larrow] (2,3) -- (2,2);
\draw [rarrow] (-2.3,3) -- (-2,2);\draw [rarrow] (-3.3,3) -- (-3,2);
\draw [rarrow] (2.3,-3) -- (2,-2);\draw [rarrow] (3.3,-3) -- (3,-2);
\draw [larrow] (-1,-3) -- (-1,-2);\draw [larrow] (-2,-3) -- (-2,-2);



% Cars
\node[inner sep=0pt] (green) at (-2.1,2.2) {\includegraphics[width=0.12\textwidth]{figures/tikz/car_fzi_green.png}};
\node[inner sep=0pt] (red) at (3.2,-2.5) {\includegraphics[width=0.14\textwidth]{figures/tikz/car_fzi_red.png}};
\node[inner sep=0pt] (yellow) at (5,1) {\includegraphics[width=0.18\textwidth]{figures/tikz/car_fzi_yelloq.png}};

    \end{tikzpicture}


==> figures/tikz/topo_model.tex <==

  \begin{tikzpicture}[
      scale=0.6,
      arrow/.style={thin,<->,shorten >=1pt,shorten <=1pt,>=stealth},
      larrow/.style={thick,<-,>=stealth},
      rarrow/.style={thick,->,>=stealth}
    ]
\draw [thick] (-7,-1.5) -- (-2.5,-1.5)node[midway,below]{$a_1$};
\draw [thick] (-7,1.5) -- (-2.5,1.5);
\draw [thick] (-7,0.5) -- (-2.5,0.5);
\draw [thick] (-7,-0.5) -- (-2.5,-0.5);
\draw [thick] (-2.5,0.5) -- (-2.5,-0.5);

\draw [thick] (7,-1.5) -- (2.5,-1.5)node[midway,below]{$a_3$};
\draw [thick] (7,1.5) -- (2.5,1.5) node (origo) {};
\draw [thick] (7,0.5) -- (2.5,0.5);
\draw [thin, dashed] (7,-0.5) -- (2.5,-0.5);

\draw [thick] (-2.5,-4) -- (-2.5,-1.5)node[align=center,midway,left]{$a_2$};
\draw [thin,dashed] (-1.5,-4) -- (-1.5,-1.5)  node [pos=-0.1,left]{$O_{a_2}=2$};
\draw [thick] (0.5,-4) -- (0.5,-1.5);
\draw [thick] (-0.5,-1.5) -- (0.5,-1.5);
\draw [thick] (-0.5,-4) -- (-0.5,-1.5);
\draw [thin, dashed] (1.5,-4) -- (1.5,-1.5);
\draw [thick] (2.5,-4) -- (2.5,-1.5);

\draw [thick] (-2.5,4) -- (-2.5,1.5)node[midway,left]{$a_4$};
\draw [thin,dashed] (-1.5,4) -- (-1.5,1.5)node[pos=-0.1,left]{$E_{a_4}=2$};
\draw [thick] (-0.5,1.5) -- (1.5,1.5);
\draw [thick] (-0.5,4) -- (-0.5,1.5);
\draw [thick] (1.5,4) -- (1.5,1.5);
\draw [thick] (2.5,4) -- (2.5,1.5)node (beta) {};

\tkzDefPoint(0,1){C}
\tkzDefPoint(0,0){B}
\tkzDefPoint(1,0){A}
\pic [draw, <-, angle radius=8mm, angle eccentricity=0.6, "$\alpha_{3}$"] {angle = A--B--C};

\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-7,-0.5) rectangle (-2.5,0.5);
\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-0.5, -4) rectangle (0.5, -1.5);
\draw[opacity=0.1, draw=none, pattern=north west lines, pattern color=black] (-0.5, 4) rectangle (1.5, 1.5);

%% Trajectories
%\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-yellow] (2,4) -- (2, 1.5) -- (2.15, 1.15) -- (2.5, 1) -- (7, 1);
%\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-lightblue] (7,-1) -- (-7, -1);
%\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-red] (2,-4) -- (2, 4);
%\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-happygreen] (-1,4) -- (-1, -4);

% Arrows
\draw [arrow] (-0.5,3) -- (1.5,3)node[midway,below]{$g_{a_4}$};
\draw [arrow] (-7.5,-0.5) -- (-7.5,-1.5)node[align=center,midway,left]{$w$};
%\draw [rarrow] (0,0) -- (0,1)node[midway,right]{$d_{a_4}$}; % TODO: what is param d?

\draw [rarrow] (-5,-1) -- (-4,-1);\draw [larrow] (-5,1) -- (-4,1);
\draw [larrow] (5,-1) -- (4,-1);\draw [rarrow] (5,1) -- (4,1);
\draw [larrow] (5,0) -- (4,0);

\draw [larrow] (2,3) -- (2,2);
\draw [rarrow] (-1,3) -- (-1,2);\draw [rarrow] (-2,3) -- (-2,2);
\draw [rarrow] (1,-3) -- (1,-2);\draw [rarrow] (2,-3) -- (2,-2);
\draw [larrow] (-1,-3) -- (-1,-2);\draw [larrow] (-2,-3) -- (-2,-2);

\draw [rarrow] (0,0) -- (0,1);
\draw [rarrow] (0,0) -- (1,0);
\filldraw (0,0) circle (2pt) node[align=right,below] {$c$};


%% Cars
%\node[inner sep=0pt] (green) at (-1.1,2.2) {\includegraphics[width=0.12\textwidth]{figures/tikz/car_fzi_green.png}};
%\node[inner sep=0pt] (red) at (2,-2.5) {\includegraphics[width=0.14\textwidth]{figures/tikz/car_fzi_red.png}};
%\node[inner sep=0pt] (yellow) at (4,1) {\includegraphics[width=0.18\textwidth]{figures/tikz/car_fzi_yelloq.png}};

\end{tikzpicture}


==> figures/tikz/topo_model_withtraj.tex <==

\begin{tikzpicture}[
scale=0.6,
arrow/.style={thin,<->,shorten >=1pt,shorten <=1pt,>=stealth},
larrow/.style={thick,<-,>=stealth},
rarrow/.style={thick,->,>=stealth}
]

% Intersection
\draw [thick] (-7,-1.5) -- (-2.5,-1.5);
\draw [thick] (-7,1.5) -- (-2.5,1.5);
\draw [thick] (-7,0.5) -- (-2.5,0.5);
\draw [thick] (-7,-0.5) -- (-2.5,-0.5);
\draw [thick] (-2.5,0.5) -- (-2.5,-0.5);

\draw [thick] (7,-1.5) -- (2.5,-1.5);
\draw [thick] (7,1.5) -- (2.5,1.5) node (origo) {};
\draw [thick] (7,0.5) -- (2.5,0.5);
\draw [thin, dashed] (7,-0.5) -- (2.5,-0.5);

\draw [thick] (-2.5,-4) -- (-2.5,-1.5);
\draw [thin,dashed] (-1.5,-4) -- (-1.5,-1.5);
\draw [thick] (0.5,-4) -- (0.5,-1.5);
\draw [thick] (-0.5,-1.5) -- (0.5,-1.5);
\draw [thick] (-0.5,-4) -- (-0.5,-1.5);
\draw [thin, dashed] (1.5,-4) -- (1.5,-1.5);
\draw [thick] (2.5,-4) -- (2.5,-1.5);

\draw [thick] (-2.5,4) -- (-2.5,1.5);
\draw [thin,dashed] (-1.5,4) -- (-1.5,1.5);
\draw [thick] (-0.5,1.5) -- (0.5,1.5);
\draw [thick] (-0.5,4) -- (-0.5,1.5);
\draw [thick] (1.5,4) -- (1.5,1.5);
\draw [thick] (0.5,4) -- (0.5,1.5);
\draw [thick] (2.5,4) -- (2.5,1.5)node (beta) {};


% Areas
\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-7,-0.5) rectangle (-2.5,0.5);
\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-0.5, -4) rectangle (0.5, -1.5);
\draw[opacity=0.1, draw=none, pattern=north west lines, pattern color=black] (-0.5, 4) rectangle (0.5, 1.5);

% Arrows
\draw [rarrow] (-5,-1) -- (-4,-1);\draw [larrow] (-5,1) -- (-4,1);
\draw [larrow] (5,-1) -- (4,-1);\draw [rarrow] (5,1) -- (4,1);
\draw [larrow] (5,0) -- (4,0);

\draw [larrow] (2,3) -- (2,2);
\draw [larrow] (1,3) -- (1,2);
\draw [rarrow] (-1,3) -- (-1,2);\draw [rarrow] (-2,3) -- (-2,2);
\draw [rarrow] (1,-3) -- (1,-2);\draw [rarrow] (2,-3) -- (2,-2);
\draw [larrow] (-1,-3) -- (-1,-2);\draw [larrow] (-2,-3) -- (-2,-2);
\filldraw (0,0) circle (2pt);

% Trajectories
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-yellow] (2,4) -- (2, 1.5) -- (2.15, 1.15) -- (2.5, 1) -- (7, 1);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-lightblue] (7,-1) -- (-7, -1);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-red] (2,-4) -- (2, 4);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-happygreen] (-1,4) -- (-1, -4);

% Cars
\node[inner sep=0pt] (green) at (-1.1,2.2) {\includegraphics[width=0.12\textwidth]{figures/tikz/car_fzi_green.png}};
\node[inner sep=0pt] (red) at (2,-2.5) {\includegraphics[width=0.14\textwidth]{figures/tikz/car_fzi_red.png}};
\node[inner sep=0pt] (yellow) at (4,1) {\includegraphics[width=0.18\textwidth]{figures/tikz/car_fzi_yelloq.png}};


\end{tikzpicture}


==> figures/tikz/topo_model_withtraj_split_concept.tex <==

\begin{tikzpicture}[
scale=0.6,
arrow/.style={thin,<->,shorten >=1pt,shorten <=1pt,>=stealth},
larrow/.style={thick,<-,>=stealth},
rarrow/.style={thick,->,>=stealth}
]
\draw [thick] (-7,-1.5) -- (-2.5,-1.5);
\draw [thick] (-7,1.5) -- (-2.5,1.5);
\draw [thick] (-7,0.5) -- (-2.5,0.5);
\draw [thick] (-7,-0.5) -- (-2.5,-0.5);
\draw [thick] (-2.5,0.5) -- (-2.5,-0.5);

\draw [thick] (7,-1.5) -- (2.5,-1.5);
\draw [thick] (7,1.5) -- (2.5,1.5) node (origo) {};
\draw [thick] (7,0.5) -- (2.5,0.5);
\draw [thin, dashed] (7,-0.5) -- (2.5,-0.5);

\draw [thick] (-2.5,-4) -- (-2.5,-1.5);
\draw [thin,dashed] (-1.5,-4) -- (-1.5,-1.5);
\draw [thick] (0.5,-4) -- (0.5,-1.5);
\draw [thick] (-0.5,-1.5) -- (0.5,-1.5);
\draw [thick] (-0.5,-4) -- (-0.5,-1.5);
\draw [thin, dashed] (1.5,-4) -- (1.5,-1.5);
\draw [thick] (2.5,-4) -- (2.5,-1.5);

\draw [thick] (-2.5,4) -- (-2.5,1.5);
\draw [thin,dashed] (-1.5,4) -- (-1.5,1.5);
\draw [thick] (-0.5,1.5) -- (0.5,1.5);
\draw [thick] (-0.5,4) -- (-0.5,1.5);
\draw [thick] (1.5,4) -- (1.5,1.5);
\draw [thick] (0.5,4) -- (0.5,1.5);
\draw [thick] (2.5,4) -- (2.5,1.5)node (beta) {};

% Tunnels
\fill[fzi-lightblue, nearly transparent]  (-7,-1.5) -- (-7,-0.5) -- (-0.3,-0.5) -- (-0.3,-1.5) -- cycle;
\draw[fzi-lightblue, thick]  (-7,-1.5) -- (-7,-0.5) -- (-0.3,-0.5) -- (-0.3,-1.5) -- cycle;
%\draw[fzi-lightblue, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round] (-1,-1) --(1,-1);
\fill[fzi-lightblue, nearly transparent]  (0.3,-1.5) -- (0.3,-0.5) -- (7,-0.5) -- (7,-1.5) -- cycle;
\draw[fzi-lightblue, thick]  (0.3,-1.5) -- (0.3,-0.5) -- (7,-0.5) -- (7,-1.5) -- cycle;
\node  at (-5, -2) {$e_1$};
\node  at (5, -2) {$o_1$};

\fill[fzi-red, nearly transparent]  (1.5,-4) -- (1.5,-0.3) -- (2.5,-0.3) -- (2.5,-4) -- cycle;
\draw[fzi-red, thick]  (1.5,4) -- (1.5,0.3) -- (2.5,0.3) -- (2.5,4) -- cycle;
%\draw[fzi-red, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round] (2,-1) --(2,1);
\fill[fzi-red, nearly transparent]  (1.5,4) -- (1.5,0.3) -- (2.5,0.3) -- (2.5,4) -- cycle;
\draw[fzi-red, thick]  (1.5,-4) -- (1.5,-0.3) -- (2.5,-0.3) -- (2.5,-4) -- cycle;
\node  at (3, -3) {$e_2$};

\fill[fzi-happygreen, nearly transparent]  (-0.5,-4) -- (-0.5,-0.3) -- (-1.5,-0.3) -- (-1.5,-4) -- cycle;
\draw[fzi-happygreen, thick]  (-0.5,-4) -- (-0.5,-0.3) -- (-1.5,-0.3) -- (-1.5,-4) -- cycle;
%\draw[fzi-happygreen, dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round] (-1,-1) --(-1,1);
\fill[fzi-happygreen, nearly transparent]  (-0.5,0.3) -- (-0.5,4) -- (-1.5,4) -- (-1.5,0.3) -- cycle;
\draw[fzi-happygreen, thick]  (-0.5,0.3) -- (-0.5,4) -- (-1.5,4) -- (-1.5,0.3) -- cycle;
\node  at (-0.1, -3) {$o_4$};
\node  at (-0.1, 3) {$e_4$};

\fill[fzi-yellow, nearly transparent] (2.8, 0.5) -- (7, 0.5) -- (7,1.5) -- (2.8,1.5) -- cycle;
\draw[fzi-yellow, thick] (2.8, 0.5) -- (7, 0.5) -- (7,1.5) -- (2.8,1.5) -- cycle;
%\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round,  orange] (2, 2) -- (2,1.5) -- (3,1) -- (3.5, 1);
\fill[fzi-yellow, nearly transparent] (1.5,4) -- (1.5, 1.5) -- (2.5, 1.5) -- (2.5,4) --  cycle;
\draw[fzi-yellow, dashed, thick] (1.5,4) -- (1.5, 1.5) -- (2.5, 1.5) -- (2.5,4) --  cycle;
\node  at (5, 2) {$e_3$};
\node  at (3.5, 3) {$o_2/o_3$};

% Trajectories
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-yellow] (2,4) -- (2, 1.5) -- (2.15, 1.15) -- (2.5, 1) -- (7, 1);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-lightblue] (7,-1) -- (-7, -1);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-red] (2,-4) -- (2, 4);
\draw [dash pattern=on \pgflinewidth off 5pt, line width=3pt, line cap=round, fzi-happygreen] (-1,4) -- (-1, -4);

% Dashed Areas
\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-7,-0.5) rectangle (-2.5,0.5);
\draw[opacity=0.2, draw=none, pattern=north west lines, pattern color=black] (-0.5, -4) rectangle (0.5, -1.5);
\draw[opacity=0.1, draw=none, pattern=north west lines, pattern color=black] (-0.5, 4) rectangle (0.5, 1.5);

% Arrows
\draw [rarrow] (-5,-1) -- (-4,-1);\draw [larrow] (-5,1) -- (-4,1);
\draw [larrow] (5,-1) -- (4,-1);\draw [rarrow] (5,1) -- (4,1);
\draw [larrow] (5,0) -- (4,0);

\draw [larrow] (2,3) -- (2,2);
\draw [larrow] (1,3) -- (1,2);
\draw [rarrow] (-1,3) -- (-1,2);\draw [rarrow] (-2,3) -- (-2,2);
\draw [rarrow] (1,-3) -- (1,-2);\draw [rarrow] (2,-3) -- (2,-2);
\draw [larrow] (-1,-3) -- (-1,-2);\draw [larrow] (-2,-3) -- (-2,-2);
\filldraw (0,0) circle (2pt);

\end{tikzpicture}

